Detecting Robustness against MVRC for Transaction Programs with Predicate Reads

The transactional robustness problem revolves around deciding whether, for a given workload, a lower isolation level than Serializable is sufficient to guarantee serializability. The paper presents a new characterization for robustness against isolation level (multi-version) Read Committed. It supports transaction programs with control structures (loops and conditionals) and inserts, deletes, and predicate reads -- scenarios that trigger the phantom problem, which is known to be hard to analyze in this context. The characterization is graph-theoretic and not unlike previous decision mechanisms known from the concurrency control literature that database researchers and practicians are comfortable with. We show experimentally that our characterization pushes the frontier in allowing to recognize more and more complex workloads as robust than before.

==> smallbank-sg.tex <==
% !TeX root = main.tex
\begin{figure}
\begin{minipage}[t]{.99\linewidth}
\resizebox{.7\textwidth}{!}{
\input{tikz_auctionn_horizontal.tex}
} %\resizebox
\end{minipage}
\vspace{-3em}

\begin{minipage}[t]{.35\linewidth}
\resizebox{1\textwidth}{!}{
\input{tikz_smallbank_sg_reduced.tex}
} %\resizebox
\end{minipage}%
\hfill%
\begin{minipage}[t]{.65\linewidth-2ex}
\resizebox{1\textwidth}{!}{
\input{tikz_tpcc_sg_reduced.tex}
}
\end{minipage}

    \caption{{\emph{(top)} Auction($n$), \emph{(left)} SmallBank and \emph{(right)} TPC-C summary graphs} (no edge labels).}
    % \caption{Summary graph for the SmallBank benchmark. Counterflow edges are represented by dashed edges. To facilitate the presentation, edge labels are not visualized.}
\label{fig:smallbank:sg}
\end{figure}


% \begin{figure}
%     \begin{minipage}[t]{.99\linewidth}
%     \resizebox{1\textwidth}{!}{
%         \input{tikz_tpcc_sg_reduced.tex}
% }
%     \end{minipage}

%     \caption{TPC-C summary graph (no edge labels).}
%     % \caption{Summary graph for the SmallBank benchmark. Counterflow edges are represented by dashed edges. To facilitate the presentation, edge labels are not visualized.}
% \label{fig:tpcc:sg:small}
% \end{figure}
